Dynamic Multi-View Fusion Mechanism For Chinese Relation Extraction

Recently, many studies incorporate external knowledge into character-level feature based models to improve the performance of Chinese relation extraction. However, these methods tend to ignore the internal information of the Chinese character and cannot filter out the noisy information of external knowledge. To address these issues, we propose a mixture-of-view-experts framework (MoVE) to dynamically learn multi-view features for Chinese relation extraction. With both the internal and external knowledge of Chinese characters, our framework can better capture the semantic information of Chinese characters. To demonstrate the effectiveness of the proposed framework, we conduct extensive experiments on three real-world datasets in distinct domains. Experimental results show consistent and significant superiority and robustness of our proposed framework. Our code and dataset will be released at: https://gitee.com/tmg-nudt/multi-view-of-expert-for-chineserelation-extraction

==> Section/0-abstract.tex <==

\begin{abstract}
%== Background
% Recently, many studies incorporate external knowledge information into a model based on character input to improve the performance of Chinese relation extraction.
%
Recently, many studies incorporate external knowledge  into character-level feature based models to improve the performance of Chinese relation extraction.
%
However, these methods tend to ignore the internal information of the Chinese character and cannot filter out the  noisy information of external knowledge.
%== Method 
To address these issues, 
%
we propose  a mixture-of-view-experts framework (MoVE) to  dynamically learn multi-view features for Chinese relation extraction.
% In this framework, 
%
With  both the internal and external knowledge of Chinese characters, 
%
our framework can better capture the semantic information of Chinese characters.
%== Experiment
%
% To demonstrate the effectiveness of our method, 
To demonstrate  the effectiveness of the proposed framework,
%
% we have conducted extensive experiments on three real-world datasets in distinct domains show consistent and significant superiority and robustness of our proposed framework.
%
we conduct extensive experiments on three real-world datasets in distinct domains.
% %
Experimental results show consistent and significant superiority and robustness of our proposed
framework.
% The experimental results show that the proposed method obtains better results than state-of-the-art approaches.
%
Our code and dataset  will be released at: \url{https://gitee.com/tmg-nudt/multi-view-of-expert-for-chinese-relation-extraction}
%
\keywords{Natural Language Processing  \and Multi-view Learning \and Chinese Representation \and Chinese Relation Extraction.}
\end{abstract}

==> Section/1-Inroduction.tex <==
\section{Introduction}

% ====================  Task Background
% Information extraction (IE) aims to use natural language processing (NLP) methods to understand text semantics 
% %
% and extract useful information from unstructured texts. 
% === RESPONSE:已经修改
Information extraction (IE) is widely considered as one of the most important topics in natural language processing (NLP), 
%
which is defined as  identifying the required structured information from the unstructured texts.
%
% Relation extraction (RE) is an important task of IE. 
%
% The main purpose of RE is to identify the relations between an entity pair marked in a given sentence, and to transform unstructured text into structured data for storage.
%% === RESPONSE: 11.26修改成了关系分类的定义，但是全文并没有修改
Relation extraction (RE) has a pivotal role in information extraction, which aims to extract semantic relations between entity pairs from unstructured texts.
%
% The main purpose of RE to transform unstructured text into structured data for storage.
%
% ======================  Challenge  and Question ====
Research on Chinese RE is quite limited compared to the progress in English corpora. 
% 
% This may be due to two challenges. 
We attribute  this to the following two challenges.
% We attribute this to the two obstacles listed below.
%
First, the lack of relevant high-quality corpora  slows down the progress of research in Chinese \cite{ZiranLi2019ChineseRE,JingjingXu2017ADN}. 
%
Second, the Chinese language makes less use of function words and morphology, which makes it harder to extract semantic information from Chinese text. 
% TODO : 这个Reason 要不要说呢，下面这句话是否语气过满？
For the first challenge, existing Chinese RE datasets are subjected to sentence level or poor quality.
%
% Due to the large variances in relation type across different domains, cross-domain RE has thus far been a challenging task.
%
To tackle the first problem, we manually annotated a high-quality Chinese scientific dataset for document level RE.
%
To alleviate the issue of complex semantic representation of the Chinese language, 
%
previous research integrate the internal features (i.e. radical feature) of Chinese characters is shown to be effective for learning Chinese word embeddings \cite{JinxingYu2017JointEO,YuxianMeng2019GlyceGF}.
%
There is room for further investigation because Chinese characters have external features, which are also beneficial for improving feature representation \cite{RuotianMa2020SimplifyTU,JintongShi2022MultilevelSF}. 
%


\begin{figure}[htbp]
% \vspace{-0.8cm}
% \centering  %居中
    \subfigure[Radical View Feature.]{   %第一张子图
    \begin{minipage}{6cm}
    \centering    %子图居中
    \includegraphics[scale=0.58]{Figures/Figure1/fig1a_v2.pdf}  %以pic.jpg的0.5倍大小输出
    \label{fig:fig1a}
    \vspace{0.2cm}
    \end{minipage}
    }
    % ==============
    \subfigure[Lexicon View Feature.]{ %第二张子图
    \begin{minipage}{6cm}
    \centering    %子图居中
    \includegraphics[scale=0.58]{Figures/Figure1/fig1b_v2.pdf}
    \label{fig:fig1b}
    \vspace{0.1cm}
    \end{minipage}
    }

    
    \caption{An example of  different multi-view features in Chinese language texts.}    %大图名称
    \label{fig: fig1}    %图片引用标记
    \vspace{-0.8cm}
\end{figure}



% ====================== Internal Information [radical + semantic + char]
In Chinese texts, a sentence contains semantic information from different view features including character, morphology, word and contextual text. 
%
For example, we can encode the structural information of the Chinese character by treating \begin{CJK}{UTF8}{gbsn}{`南'}\end{CJK} as a structure composed of \begin{CJK}{UTF8}{gbsn}{`十 冂丫二'}\end{CJK}.
% ======================
% For improving the representation of a Chinese character, 
As shown in Figure \ref{fig:fig1a},
%
% In order to encode the structure information of Chinese character,
%
existing methods introduce  radical internal semantic features as well as more semantic irrelevant sub-character component information.
%
But the semantic irrelevant sub-character component information will be noisy for representing a Chinese character \cite{JinxingYu2017JointEO,JintongShi2022MultilevelSF}.  
%
% ====================== ExternalWord/lexicon information

To comprehensively represent semantic information without being affected by the issue of Chinese word segmentation.
%
Some methods  are proposed to establish a model to learn both character-level and word-level features with different view granularity \cite{RuotianMa2020SimplifyTU,ShuangWu2021MECTME}.
%
However, this external word-level information is limited by the quality of domain lexicons.
%
% ======================= External Information [lexicon + Synonymous]

Moreover, existing methods suffer from the inability of discriminating the importance of the introduced knowledge, 
%
accordingly they can not filter out introduced external noisy information.

% =================== MoVE

% ========= First: 没有进行充分交互
The aforementioned methods suffer from the two issues described below.
%
Firstly, when trying to find shared information among all views to eliminate noise and redundancy, a common practice is to map each view into a shared sub-space. 
%
However, this procedure is always conducted independently, there is no interaction among different feature view. 
%
It is difficult to guarantee that all common semantic information is adequately exploited.
% ============= Second： 无法进行动态组合
%
Second, the underlying fact that each view contains its own specific contribution to the semantic representation is ignored.
%
Existing models introduce more external knowledge as well as more noisy information, 
%
and they suffer from the inability of discriminating the importance of the multi-view features and filtering out the noisy information.
%
Is there any other better way  to fuse multi-view representation  of Chinese characters? 
%
Inspired by mixture-of-experts \cite{NoamShazeer2017OutrageouslyLN,JiaqiMa2018ModelingTR}, 
%
% in this paper,
%
we propose a novel Mixture-of-View-Experts (MoVE) model to dynamically fuse both internal and external features for Chinese RE. 
%
As shown in Figure \ref{fig:fig2},
%
MoVE is an approach for conditionally computing feature representation, given several view expert inputs, which can be models using different knowledge sources.
%
In addition, a gating network is developed to dynamically weight experts per instance based on the input.
%
In this way, the knowledge from different view experts is incorporated to model the inherent ambiguity and enhance the ability to generalize to specific domains.

%===: RESPONSE: lack experimental introduction
Moreover,

we manually annotated a high-quality Chinese scientific dataset for document level RE.
%
Extensive experiments are performed on three representative dataset across different domain,
%
and our framework consistently shows improvements over the baseline systems.

% ===================== Result & Contribu
In this paper, we propose a novel multi-view features fusion model which leverages both internal and external knowledge.
%
The main contributions of this paper can be summarized as follows:
\begin{compactitem}
    \item We propose a new Chinese scientific dataset for document-level relation extraction.
    \item According to the multi-view feature of Chinese characters, we propose a novel MoVE method to dynamically learn the representation for Chinese relation extraction. 
    \item The effectiveness of the proposed model is evaluated on three real-world Chinese relation extraction datasets from distinct domains.
\end{compactitem}
  


==> Section/1-Introduction_v1.tex <==
\section{Introduction}

% ====================  Task Background

Information extraction (IE) is widely considered as one of the most important topics in natural language processing (NLP), 
%
which is defined as  identifying the required structured information from the unstructured texts.
%
Relation extraction (RE) has a pivotal role in information extraction, which aims to extract semantic relations between entity pairs from unstructured texts.
%
%
% ======================  Challenge  and Question ====
%
Recently, deep learning-based models have obtained tremendous success in this task.
%
However, research on Chinese RE is quite limited compared to the progress in English corpora. 
%
We attribute  this to the following main challenge:
%
it is hard to extract semantic information from Chinese texts for the Chinese
language makes less use of function words and morphology.
%
Although there has been extensive previous work integrating the external knowledge (i.e. lexicon feature) of Chinese characters is shown to be effective for sequence labeling tasks \cite{JinxingYu2017JointEO,YuxianMeng2019GlyceGF,RuotianMa2020SimplifyTU,JintongShi2022MultilevelSF},
%
% There is room for further investigation to  exploit the internal features of Chinese characters.
there is room for further investigation to leverage the internal characteristics of Chinese characters.
%
% We attribute  this to the following two challenges.
% %
% % First, the lack of relevant high-quality corpora  slows down the progress of research in Chinese \cite{ZiranLi2019ChineseRE,JingjingXu2017ADN}. 
% %
% (1) lacking high-quality Chinese RE corpora \cite{ZiranLi2019ChineseRE,JingjingXu2017ADN}.
% %
% Existing Chinese RE datasets are limited to sentence level or poor quality.
%
% Second, the Chinese language makes less use of function words and morphology, which makes it harder to extract semantic information from Chinese text \cite{RuotianMa2020SimplifyTU,JintongShi2022MultilevelSF}.
% (2) it is hard to extract semantic information from Chinese texts for the Chinese
% language makes less use of function words and morphology.
%
% Although there has been extensive previous work integrate the different granularity features (i.e. lexicon feature) of Chinese characters is shown to be effective for sequence labeling tasks \cite{JinxingYu2017JointEO,YuxianMeng2019GlyceGF,RuotianMa2020SimplifyTU,JintongShi2022MultilevelSF}.
% %
% There is room for further investigation to  exploit the internal and external features of Chinese characters.
%
% ================= 
% TODO : 这个Reason 要不要说呢，下面这句话是否语气过满？
% For the first challenge, existing Chinese RE datasets are subjected to sentence level or poor quality.
% %
% To tackle the first problem, we manually annotated a high-quality Chinese scientific dataset for document level RE.
% %
% To alleviate the issue of complex semantic representation of the Chinese language, 
% %
% previous research integrate the internal features (i.e. radical feature) of Chinese characters is shown to be effective for learning Chinese word embeddings \cite{JinxingYu2017JointEO,YuxianMeng2019GlyceGF}.
% %
% There is room for further investigation because Chinese characters have external features, which are also beneficial for improving feature representation \cite{}. 



% ====================== Internal Information [radical + semantic + char]
In Chinese texts, a sentence contains semantic information from different view features including character, word, structure and contextual semantic information. 
% ====================== ExternalWord/lexicon information External Information [lexicon + Synonymous]
% To represent semantic information without being affected by the issue of Chinese word segmentation.
As shown in Figure \ref{fig:fig1a},  in order to reduce segmentation errors and increasing the semantic and boundary information of Chinese characters,
%
% some methods  are proposed to establish a model to learn both character-level and word-level features with different input granularity \cite{RuotianMa2020SimplifyTU,ShuangWu2021MECTME}.
%
some methods  are proposed to establish a model to learn both character-level and word-level features \cite{RuotianMa2020SimplifyTU,ShuangWu2021MECTME}.
%
However, this external knowledge information is limited by the quality of domain lexicons and will inevitably introduce redundant noise.
%
% For example, \begin{CJK}{UTF8}{gbsn}{`南京}\end{CJK}(Nanjing)',\begin{CJK}{UTF8}{gbsn}{`市长}\end{CJK}(Mayor)' and  \begin{CJK}{UTF8}{gbsn}{`南京市}\end{CJK}(Nanjing City)',\begin{CJK}{UTF8}{gbsn}{`长江}\end{CJK}(YangZi River)'  only one applicable semantic information is allowed.
%
For example, only one of \begin{CJK}{UTF8}{gbsn}{`南京}\end{CJK}(Nanjing)',\begin{CJK}{UTF8}{gbsn}{`市长}\end{CJK}(Mayor)' and  \begin{CJK}{UTF8}{gbsn}{`南京市}\end{CJK}(Nanjing City)',\begin{CJK}{UTF8}{gbsn}{`长江}\end{CJK}(YangZi River)' is an appropriate contextual information.
%
\begin{figure}[htbp]
\vspace{-0.51cm}
% \centering  %居中
    \subfigure[The lexicon view feature.]{ %第二张子图
    \begin{minipage}{6cm}
    \centering    %子图居中
    \includegraphics[scale=0.58]{Figures/Figure1/fig1b_v3.pdf}
    \label{fig:fig1a}
    \vspace{0.1cm}
    \end{minipage}
    }
    \subfigure[The radical view feature.]{   %第一张子图
    \begin{minipage}{6cm}
    \centering    %子图居中
    \includegraphics[scale=0.58]{Figures/Figure1/fig1a_v2.pdf}  %以pic.jpg的0.5倍大小输出
    \label{fig:fig1b}
    \vspace{0.2cm}
    \end{minipage}
    }
    % ==============

    \caption{An example of multi-view features in Chinese language texts.}   
    \label{fig: fig1}    %图片引用标记
    \vspace{-0.8cm}
\end{figure}
%
% Moreover, existing methods suffer from the inability of discriminating the importance of the introduced knowledge, 
% %
% accordingly they can not filter out introduced external noisy information.
%
In addition, 
%
Chinese characters have evolved from pictographs since ancient times, and their structures often reflect more information about the characters.
%
The internal character structures  can enrich the semantic representation of Chinese characters.
%
%
As shown in Figure \ref{fig:fig1b}, \begin{CJK}{UTF8}{gbsn}{`氵'}\end{CJK}  is the radical of  \begin{CJK}{UTF8}{gbsn}{`江(River)'}\end{CJK}, and suggests \begin{CJK}{UTF8}{gbsn}{`氵(water)'}\end{CJK} that river is water-like liquid.
% As shown in Figure \ref{fig:fig1b}, we can encode the structural information of the Chinese character by treating \begin{CJK}{UTF8}{gbsn}{`江'}\end{CJK} as a structure composed of \begin{CJK}{UTF8}{gbsn}{`氵工'}\end{CJK}.
% ======================
%
% However, existing methods introduce  radical internal semantic features as well as more semantic irrelevant sub-character component information \cite{YuxianMeng2019GlyceGF,ShuangWu2021MECTME}.
% However,
On the contrary,
%
the \begin{CJK}{UTF8}{gbsn}{`南(south)'}\end{CJK}  can be encoded as a structure consisting of \begin{CJK}{UTF8}{gbsn}{`十', `冂', `丫', and `二'}\end{CJK}, but they convey no meaningful semantic information.
%
Previous studies have proven that
%
semantic irrelevant sub-character component information will be noisy for representing a Chinese character \cite{JinxingYu2017JointEO,JintongShi2022MultilevelSF}.  
%
% =================== MoVE
%
% Although these methods have achieved reasonable performance, they suffer from the common issues described below.
Although above methods have achieved reasonable performance, they still suffer from two common issue:
% The aforementioned methods suffer from the two  common issues described below.
%
(1) The underlying fact that different view feature contains its own specific contribution to the semantic representation is ignored.
%
Existing methods map different view features into a shared space without interaction among views, which is difficult to guarantee that all common semantic information is adequately exploited.
%
(2) Existing methods introduce external knowledge as well as more noisy information, 
%
and they suffer from the inability of discriminating the importance of the different features and filtering out the noisy information.
%


% ========= First: 没有进行充分交互
% The aforementioned methods suffer from the two  common issues described below.
% %
% Firstly, when trying to find shared information among all views to eliminate noise and redundancy, a common practice is to map each view into a shared space. 
% %
% However, this procedure is always conducted independently, there is no interaction among different feature view. 
% %
% It is difficult to guarantee that all common semantic information is adequately exploited.
% ============= Second： 无法进行动态组合
%
% Second, the underlying fact that each view contains its own specific contribution to the semantic representation is ignored.
%
% Existing models introduce more external knowledge as well as more noisy information, 
% %
% and they suffer from the inability of discriminating the importance of the multi-view features and filtering out the noisy information.
%
Is there any other better way  to fuse multi-view features of Chinese characters? 
%
Inspired by mixture-of-experts \cite{NoamShazeer2017OutrageouslyLN,JiaqiMa2018ModelingTR,ZihanLiu2020ZeroResourceCN},
%
%
we propose a novel Mixture-of-View-Experts (MoVE) model to dynamically fuse both internal and external features for Chinese RE. 
%
As shown in Figure \ref{fig:fig2},
%
% MoVE is an approach for conditionally computing feature representation, given several view expert inputs, which can be models using different knowledge sources.
%
MoVE is a method for conditionally computing feature representation, given multiple view expert inputs that can be represented utilizing diverse knowledge sources.
%
% In addition, a gating network is designed to dynamically calculate each expert weight experts per instance based on the input.
%
In addition, a gating network is designed to dynamically calculate each expert weight per instance based on the multi-view
feature.
%
In this way, the knowledge from different view experts can be incorporated to model the inherent ambiguity and enhance the ability to generalize to specific domains.
%
%===: RESPONSE: lack experimental introduction
% Moreover,
% %
% to alleviate the issue of dataset scarcity and promote Chinese RE research,
%
% we manually annotated a high-quality Chinese scientific dataset for document level RE.
%
Extensive experiments are conducted on three representative datasets across different domains,
%
%
% and our framework consistently shows improvements over the baseline systems.
Experimental results show that our framework consistently improves the selected baselines


% ===================== Result 
In this paper, we propose a novel multi-view features fusion framework which leverages both external and internal  knowledge.
%
The main contributions of this paper can be summarized as follows:
\begin{compactitem}
    % \item We propose a new Chinese scientific dataset for document-level relation extraction.
    \item We design a novel architecture framework capable of acquiring semantic, lexical, and radical feature information from Chinese characters.
    % \item According to the multi-view features, we propose a  MoVE method to dynamically compose the different features for Chinese relation extraction. 
    \item Based on the multi-view features, we propose the MoVE method for dynamically composing the different features for Chinese relation extraction.
    % \item The effectiveness of the proposed model is evaluated on three real-world Chinese relation extraction datasets from distinct domains.
    \item Our method achieves new state-of-the-art performance on three real-world Chinese relation extraction datasets.
\end{compactitem}
  


==> Section/2-Relatedwork.tex <==
\section{Related Work}

\subsection{Chinese Relation Extraction}
% --------------- Dataset
As a fundamental task in NLP, Relation Extraction (RE)  has been studied extensively in the past decade.
%
Here various neural network based models, such as  CNNs \cite{DaojianZeng2014RelationCV}, RNNs \cite{DongxuZhang2015RelationCV} or Transformer-based architectures \cite{ShanchanWu2019EnrichingPL} have been investigated.
%
% Research on Chinese relation extraction is quite limited compared with the progress with English. 
% % 
% This may be due to two reasons. 
% %
% First, the Chinese language makes less use of function words and morphology, which makes it harder to extract syntactic information from it. 
% %
% Second, the lack of relevant high-quality corpora  also slows down the progress of research in Chinese \cite{LiShuangjie2019DuIEAL,2017}. 
% % 
% ------------------- Model
Existing methods for Chinese RE are mostly character-based or word-based implementations of mainstream NRE models. 
%
In most cases, these methods only focus on the improvement of the model itself, 
%
ignoring the fact that different granularity of input will have a significant impact on the RE models. \cite{ZiranLi2019ChineseRE,JingjingXu2017ADN,QianqianZhang2018AnEG}.
%
The character-based model can not utilize the information of words, capturing fewer features than the word-based model. 
%
On the other side, the performance of the word-based model is significantly impacted by the quality of segmentation \cite{YueZhang2018ChineseNU}. 
%
Then, lexicon enhanced methods are used to combine character-level and word-level information in other NLP tasks like character-bigrams 
%
and lexicons information \cite{XiaotangZhou2022DynamicMF,HengDaXu2021ReadLA,BaojunWang2021DyLexID}.
%
Although, lexicon enhanced models can exploit char and external lexicon information, it still could be severely affected by the ambiguity of polysemy.
%
Therefore,
%
We utilize external linguistic knowledge  with the help of HowNet \cite{ZhendongDong2003HowNetA}, which is a concept knowledge base that annotates Chinese with correlative word synonyms.
%
% In this paper, We proposed xxxx




\subsection{Chinese Character Representation}
%
Existing  models of Chinese character representation can be divided into two categories: 
%
exploiting the structural information of the characters themselves and injecting external knowledge.
% -------------------- Internal View Feature
% Chinese characters are often composed of subcharacter components which are also semantically informative, 
% %
% and the component-level internal semantic features of a Chinese character inherently bring with additional information.
%
% Therefore, there have been several studies that utilized subcharacter component information (e.g. radical, fine-grained components and stroke n-grams) to improve Chinese character representation.
% ===
%
JWE \cite{JinxingYu2017JointEO} is introduced to jointly learn Chinese component, character and word embeddings, which takes character information for improving the quality of word embeddings. 
%
LSN \cite{YanSong2018JointLE} is proposed to capture the relations among radicals, characters and words of Chinese and learn their embeddings synchronously.
%
CW2VEC \cite{CaoShaosheng2018cw2vecLC} adopts the stroke n-gram of Chinese words and utilizes the fine-grained information associated with word semantics to learn Chinese word embeddings.
% --------------------External  View Feature
% In order to exploring the internal semantic characteristics of subcharacter component, 
% %
% the recent studies have also been conducted to obtain semantic representations by integrating external linguistic knowledge.
% lexicon 
In order to effectively leverage the external word semantic and enhance character boundary representation, a few models aimed to integrate lexicon information into character-level sequence labeling \cite{RuotianMa2020SimplifyTU,YueZhang2018ChineseNU,BaojunWang2021DyLexID,CanwenXu2019ExploitingME}.
% morphay
Besides, there are models  utilize sense-level information with external sememe-based lexical knowledge base
%
,to handle the polysemy of words with the change of language situation \cite{ZiranLi2019ChineseRE,ZhendongDong2003HowNetA,FanchaoQi2019OpenHowNetAO}.


\subsection{Multi-View Learning}

There has been some research to integrate information from different multi-view to achieve better performance. 
% ================== interaction fusion 
% In order to incorporate the visual information of Chinese characters into language models, 
%
ME-CNER \cite{CanwenXu2019ExploitingME} concatenates the character embeddings in radical, character and word levels to form the final character representation, which exploits multiple embeddings together in different granularities for Chinese NER.  
% 
To fully explore the contribution of each view embedding,  FGAT \cite{XiaosuWang2021ImprovingCC} is proposed to discriminate the importance of the different granularities internal semantic features with the help of graph attention network.
%
ReaLiSe \cite{HengDaXu2021ReadLA}  leverages the semantic, phonetic and graphic information to tackle Chinese Spell Checking (CSC) task,  which introduce the selective fusion mechanism base Transformer \cite{AshishVaswani2017AttentionIA} to integrate multi-view information.
%
Recent, some efforts incorporate both internal and external multi-view information (such as lattice, glyce, pinyin, n-gram information ) with the character token in Chinese Pre-trained language models (PLMs) and design specific pre-train task \cite{ZijunSun2021ChineseBERTCP,QianglongChen2022DictBERTDD,YuxuanLai2021LatticeBERTLM}.
%
To the best of our knowledge, this paper is the first work to leverage multi-view information to tackle the Chinese Relation Extraction task.

% % =================== multimodal 
% %
% Tasks such as Multimodal Sentiment Analysis (Zadeh et al., 2016; Zhang et al., 2019),
% Visual Question Answering (Antol et al., 2015;
% Chao et al., 2018) and Multimodal Machine Translation (Hitschler et al., 2016; Barrault et al., 2018) have made much progress. 
% % 
% Recently, multimodal pretraining models have been proposed, such as
% VL-BERT (Su et al., 2020), Unicoder-VL (Li et al.,
% 2020), and LXMERT (Tan and Bansal, 2019). 



==> Section/3-Method.tex <==
\section{Methodology}

%Given a Chinese sentence and two marked entities in it, the task of Chinese relation extraction is to extract semantic relations between the two entities. 
%
An overview of the proposed MoVE framework is depicted in Figure \ref{fig:fig2}.
%
In this section,
% we first formally define the Chinese relation extraction task,
%
% and then
we introduce our model architecture from three perspectives: Multi-View Features Representation, Mixture-of-View-Expert, 
and Relation Classifier.
%
%

% Overview

% \subsection{Problem Definition}
% % Problem Define 
% In this paper, we focus on Chinese Relation Extraction (RE). 
% %
% Specifically, given a Chinese sentence $X = (x_1, x_2, x_3, \dots, x_n)$ mentioning an entity pair $(e_s, e_o)$, referred as the subject and object entities,
% %
% respectively, the task of  RE is to predict the relationship $r$ between $e_s$ and $e_o$ from R$\cup$NA, where R is a pre-defined set of relationships of interest. 
% %
% If the text does not express any relation from R, the entity pair will be accordingly labeled NA.


\begin{figure}
    % \centering
    \includegraphics[scale=0.68]{Figures/Figure2/fig2v7.pdf}
    \caption{The architecture of  our MoVE framework. }
    \label{fig:fig2}
    \vspace{-0.3cm}
\end{figure}

\subsection{Multi-View Features Representation}
\subsubsection{Internal View Feature \newline} 
% ========================= Semantic Embeddings
\hspace{5pt} \textbf{Semantic Embeddings}
%
We adopt BERT  \cite{JacobDevlin2022BERTPO} as the backbone of the semantic encoder. 
%
BERT provides rich contextual word representation with the unsupervised pretraining on large corpora and has been proven superior in building contextualized representations for various NLP tasks \cite{ZiranLi2019ChineseRE,HengDaXu2021ReadLA,JacobDevlin2022BERTPO,TongfengGuan2020CMeIECA}. 
%
% The input tokens  $X = (x_1, x_2, x_3, \dots, x_n)$ are first projected into $H^t_0$ through the input embedding. 
Hence, we utilize  BERT as the underlying encoder to yield the basic contextualized character representations.
%
The output of the last layer  $H^c_{i}$  is used as the contextualized semantic embeddings of Chinese characters at the semantic view.
\begin{equation*}
    H^c_i = \mbox{BERT} (x_1, x_2, x_3, \dots, x_n)
\end{equation*}
%

% ===================== Radical Embeddings
\textbf{Radical Embeddings}  
%
Chinese characters are based on pictographs, and their meanings are expressed in the shape of objects.
%
The radical is often the semantic component and inherently bring with certain levels of semantics regardless of the contexts.
%
In this case, the internal structure of Chinese characters has certain useful information.
%
For example, the radicals such as \begin{CJK}{UTF8}{gbsn}{`月'}\end{CJK} (body) represents human body parts or organs, and \begin{CJK}{UTF8}{gbsn}{`疒'}\end{CJK}  (disease) represents diseases, which benefits Chinese  RE for the medical field.
%
We choose the  informative Structural Components (SC)  as radical-level features of Chinese characters, which comes from the online XinHua Dictionary\footnote{\url{https://github.com/kfcd/chaizi}}. 
%
Specifically, we first disassemble the Chinese characters  into $SC=(x^{c_1}_1,x^{c_2}_1, x^{c_3}_1, \dots, x^{c_i}_n )$, and then input the radical features into CNN. 
%
For example, we can decompose  \begin{CJK}{UTF8}{gbsn}{`脚'}\end{CJK} as \begin{CJK}{UTF8}{gbsn}{`月土厶卩'}\end{CJK}, 
\begin{CJK}{UTF8}{gbsn}{`疼'}\end{CJK} as \begin{CJK}{UTF8}{gbsn}{ `疒夂丶丶'}\end{CJK}.
%
Then, we use the max-pooling and fully connection layers to get the feature embedding $H^r_i$ of Chinese characters at the radical view.
%
\begin{equation*}
    H^r_i = \mbox{Max-Pooling}(\mbox{CNN} (x^{c_1}_1,x^{c_2}_1, x^{c_3}_1, \dots, x^{c_i}_n ))
\end{equation*}
%
\vspace{-1cm}
\subsubsection{External View Feature \newline}  
% ===============================
\hspace{5pt} \textbf{Lexicon Embeddings}
%
Recently, lexical enhancement methods were proposed to enhance character-based models, which have demonstrated the benefits of integrating information from external lexicons for Chinese NER tasks.
%
Following SoftLexicon \cite{RuotianMa2020SimplifyTU}, we  retain the segmentation information, all matched words of each character $x_i$ is categorized into four word sets `BMES'.
%
After obtaining the `BMES' word sets for each character, each word set is then condensed into a fixed-dimensional vector with average-pooling method:  

\begin{equation*}
    v^s(S) = \frac{1}{|S|} \sum_{w \in S} e^w (w) 
\end{equation*}
where $S \in $ `BMES' denotes a word set and $e^w$ denotes the word embedding in external lexicon.
%
The final step is to combine the representations of four word sets into one fix-dimension feature, and concatenate them to  get the external feature embeddings $H^l_i$ of each character at the lexicon view.

\begin{equation*}
    H^l_i = \mbox{concat}(v^s(B); v^s(M); v^s(E); v^s(S))
\end{equation*}


% ===============================
% \textit{Synonyms Embeddings} 
% %
% Furthermore, the fact that Chinese words are usually ambiguous cannot be neglected, which affects the model's ability to obtain correct semantic information. 
% %
% For instance, the word \begin{CJK}{UTF8}{gbsn}{"杜 鹃"}\end{CJK}  has multiple meanings, including the ''cuckoo'' bird and the ''azalea'' flower. 
% %
% It can even be used as a given name for a person and so on. 
% %
% It is difficult to distinguish which meaning is represented in plain texts without the help of external knowledge.
% %
% %
% Therefore, we first retrieved all the external synonyms $(e_{p_1}, e_{p_2}, \cdots, e_{p_i})$ of entity $e_i$ in the orignal sentence with the help of HowNet \cite{ZhendongDong2003HowNetA}. 
% %
% Then, a cosine algorithm is designed to calculate the similarity between the external synonyms  and the original sentence for each synonym, and we select the most similar external synonym  as $Synonym(e_i)$.
% %
% Specifically, if no polysemous words are retrieved in the external knowledge base, we choose $e_i$ itself as $Synonym(e_i)$.
% %
% Finally, we combine the representations of $e_i$ and $synonym(e_i)$  to get the feature embedding $H^e_{i}$ of entity at the Synonym view.
% %
% \begin{equation}
%     Synonym(e_i) = \mathop{max}\limits_{similarity} (e_{p_1}, e_{p_2}, \cdots, e_{p_i} )
% \end{equation}

% =============================
% \textit{Pinyin Embeddings}
% todo

\vspace{-0.3cm}
\subsection{Mixture-of-View-Experts}
\vspace{-0.15cm}
%
% After applying the previously mentioned multi-view feature embeddings methods, we get two internal representation vectors $H^s_{i}$, $H^r_{i}$ in character level granularity, and  two external representations vectors $H^{l}_i$,  $H^e_{i}$ in word level granularity. 
%
% After using the aforementioned multi-view feature embeddings methods, we get both  internal  and external representation in character-level and word-level granularity.
%
After using the aforementioned multi-view feature embeddings methods, we get three representation at $h^c_i$,  $h^l_i$, $h^r_i$  in semantic-level, lexicon-level  and radical-level respectively.
%
Then we concatenate the different view features to get the multi-feature representation $h^m_i$, as shown in Figure \ref{fig:fig2}.
% ================== 从抑制噪声和效率的角度来引出MOE的动机
% 减轻Noisy label 
%
The multi-view feature representations of Chinese characters  $h^m_i$ can  capture both internal and external  features in different semantic granularity,
%
but they also introduce meaningless and noisy information simultaneously.
%
However, existing methods usually just calculate the unweighted mean of the different view features, or sometimes set the weights as hyper-parameters and calculate the weighted mean of the features \cite{RuotianMa2020SimplifyTU,XiaosuWang2021ImprovingCC}.
%
% So existing methods suffer from the inability of discriminating the importance of the introduced feature, accordingly they can not filter out introduced  potential external noisy  information \cite{XiaosuWang2021ImprovingCC,XiaotangZhou2022DynamicMF}.
%
Moreover, existing approaches are incapable of distinguishing the significance of the introduced feature. 
%
% Hence, they are unable to filter out introduced potential externally noisy information \cite{XiaotangZhou2022DynamicMF,XiaosuWang2021ImprovingCC}.
%
Hence, they are unable to filter out introduced potential noisy information \cite{XiaotangZhou2022DynamicMF,XiaosuWang2021ImprovingCC}.

%
% To allievate above mentioned issues, we design a selective fusion module based on Mixture-of-Experts (MOE) \cite{NoamShazeer2017OutrageouslyLN} mechanism to integrate these feature embeddings in different views. 
% 
% Inspired by mixture-of-experts architecture \cite{NoamShazeer2017OutrageouslyLN},
As shown in Figure \ref{fig:fig2},
%
we introduce an Mixture-of-View-Experts (MoVE) framework to combine representations generated by experts to produce the final prediction.
%
Specifically, each different feature representation acts as an view expert, which consists of two linear layers.
%
The expert gate consists of a linear layer followed by a softmax layer, which generates the confidence distribution over different view experts.
%
Finally, the meta-expert feature incorporates features from all experts based on the confidential scores from the expert gate.
%
We formulate the MoVE module as follows:

% \begin{equation*}
%     % [expt^{1}_{i}, expt^{2}_{i}, expt^{3}_{i}, expt^{4}_{i}] = [L(H_i^s), L(H_i^r), L(H_i^l), L(H^s)]
%     [expt^{1}_{i}, \cdots,  expt^{E}_{i}] = [L(h_i), \cdots, L^{E}(h_i)]
% \end{equation*}
% %
% \begin{equation*}
%     % [\alpha_1, \alpha_2, \alpha_3, \alpha_4] = Softmax(Linear(H^{t}_i))
%     [\alpha_{1}, \cdots, \alpha_{E}] = \mbox{softmax}(\mbox{Linear}(h_i))
% \end{equation*}
% %
% \begin{equation*}
% %   H^f_i = \sum_{k=1}^{4} \alpha_{k} * expt^{k}_i 
%     h^f_i = \sum_{k=1}^{E} \alpha_{k} * expt^{k}_i 
% \end{equation*}

\begin{align*}
    [expt^{1}_{i}, \cdots,  expt^{E}_{i}] &= [L(h^m_i), \cdots, L^{E}(h^m_i)] \\
    [\alpha_{1}, \cdots, \alpha_{E}] &= \mbox{softmax}(\mbox{Linear}(h^m_i)) \\
    h^f_i &= \sum_{k=1}^{E} \alpha_{k} * expt^{k}_i 
\end{align*}    
where $h^f_i$ is the meta-expert feature of $h_i$,  $expt$ is the feature derived from the expert, and L denotes the linear layer. 
%
As shown in Figure \ref{fig:fig2},
%
% We show that the MoVE has three kind experts, namely semantic, radical, and lexicon experts.
%
the MoVE has three types of experts, namely semantic, radical, and lexicon experts.
%
The expert features are computed based on the multi-view feature representations,
%
and the predictions are conditioned on the meta-expert features and the multi-view features.
%
%
% In this way, the knowledge from different view expert is incorporated to model the inherent confusion and improve the generalization ability to target domains.



\subsection{Relation Classifier}
After the MoVE model dynamically combines meta-expert feature $h^f_i$ for each token.
%
We first merge $h^f_i$ into a sentence-level feature vector $H^f$,
%
then the final sentence representation $H^f$ is  passed through  a softmax classifier to compute the confidence of each relation.
%
We formulate the classifier module as follows:

\begin{equation*}
    P(y|S) = \mbox{softmax}(W \cdot H^f + b)
\end{equation*}
%
where $W \in R^{Y \times d} $ is the transformation matrix and $b \in R^Y$ is a bias vector. $Y$ indicates the total number of relation types, and $y$ is the estimated probability for each type. 
%
% This mechanism is also applied to 
%
% Finally, given all  training examples $(S^i, y^i)$, we define the objective function using cross-entropy loss as follows:
% 
Finally, given all training examples $(S^i, y^i)$, we define the objective
function using the following cross-entropy loss:

\begin{equation*}
    \mathcal{L} (\theta) = \sum_{i=1}^{T} log P(y^i | S^i, \theta)
\end{equation*}
% where $\theta$ indicates all parameters of our model.
\vspace{-1cm}















% Addition,  we  use a pre-trained language model (e.g., BERT) to obtain contextualized representations $x_i$ for each input char $x_i$.
% % =======================
% For an entity $e_i = (x_i, x_{i+1}, \dots, x_{i+k})$,  we concatenate the Muti-View embeddings of  entity start and end tokens, and the entity length embedding as the entity representation.
% %
% The entity semantic representation $h_{e_i}$ is defined as:
% %
% \begin{equation}
%     h_{e_i} = Concat(e_{start(i)}; e_{end(i)}; \phi (e_i))
%     \label{ent_embeddings}
% \end{equation}
% %
% while $\phi(e_i)$ represents the learned embeddings of entity width features. 

% % =======================
% Given the embedding $(h_{e_s} , h_{e_o} )$ of an entity pair $(e_s, e_o)$ computed by Eq.\ref{ent_embeddings}, we map the entities to hidden states $z_s$ and $z_o$ with a linear layer followed by non-linear activation, then calculate the probability of relation $r$ by bilinear function and sigmoid activation. 
% %
% This process is formulated as:

% \begin{equation}
%     z_s = tanh(W_s h_{e_s})
% \end{equation}
% \begin{equation}
%     z_o = tanh(W_o h_{e_o})
% \end{equation}
% \begin{equation}
%   P(r| e_s,e_o) = Sigmoid (z^{t}_s W_r z_r + b_r)
% \end{equation}
% where $W_s \in R^{d \times d}, W_o \in R^{d \times d}, W_r \in R^{d \times d}, b_r \in R$ are learned model parameters. 
% %
% The representation of one entity is the same among different entity pairs.
% %
% We use the binary cross entropy loss for training. 
% %
% During inference, we tune a global threshold $\theta$ that maximizes evaluation metrics (F1 score for RE) on the development set and return $r$ as an associated relation if 
% $P (r|e_s, e_o) > \theta$ or return NA if no relation exists.

==> Section/4-Experiments.tex <==
% \newpage
\vspace{-0.3cm}
\section{Experiments}
%
\vspace{-0.15cm}
\subsection{Datasets}
%
We evaluate our approach on two popular Chinese RE datasets: FinRE \cite{ZiranLi2019ChineseRE} and  SanWen \cite{JingjingXu2017ADN}.
%
To increase domain diversity, we manually annotate the SciRE, which is the first Chinese  dataset for scientific relation extraction.
%
% DuIE \cite{LiShuangjie2019DuIEAL}, a dataset that also released in LIC2019, covers a variety of domains in real-world applications, such as news,entertainment, user-generated contents. 
% %
% The DuIE contains 49 commonly used relation types and 340,000 unique Subject-Predicate-Object (SPO) pairs. 
% %
% CMeIE \cite{TongfengGuan2020CMeIECA}, a dataset that is also released in CHIP2020, is used for Chinese medical information extraction task.
% %
% There are 53 relations defined in the CMeIE dataset, including 10 synonymous sub-relationships and 43 other sub-relationships.
%
FinRE  is a manual-labeled financial news dataset, which contains 44 distinguished relationships, including a special relation NA.
%
SanWen is a document-level Chinese literature dataset for relation extraction, including  9 relation types specific to Chinese literature articles.
%
% SciRE
% 
The SciRE dataset is collected from  3500 Chinese scientific papers in CNKI\footnote{\url{https://www.cnki.net/}},
%
which defines scientific terms and relations especially for scientific knowledge graph construction.
%
There are  4 relation types (Used-For, Compare-For, Conjunction-Of, Hyponym-Of)  defined in SciRE dataset.
% 
% We follow previous work \cite{ZiranLi2019ChineseRE} and use the same preprocessing procedure and splits for all datasets.
%
Following previous work, we use the same preprocessing procedure and splits for all datasets \cite{ZiranLi2019ChineseRE}.
%
Table \ref{tab: tab1} shows the characteristics of each dataset.

\begin{table}
\centering
\vspace{-0.8cm}
\caption{Statistics of the three experimental datasets.}
\vspace{0.2cm}
\label{tab: tab1}
\begin{tabular}{p{1.5cm}|p{1.2cm}|p{1.8cm}|p{2.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}}
% \begin{tabular}{c|c|c|c|l|l|l}
% \begin{tabular}{ccccccc}
% \hline
\toprule
    Dataset  &$\#$Type &Domain  &Characteristic  &\#Train  &\#Dev  &\#Test  \\
    % \hline
    \midrule
        \multirow{2}{*}{ \makecell{FinRE }}   
        &\multirow{2}{*}{ \makecell{44}} &\multirow{2}{*}{ \makecell{Financial}} &Sentences   &4477   &500    &1219  \\
        &                                &                                        &Triples   &9873   &1105   &2722  \\
        
    \hline 
    \specialrule{0em}{1pt}{1pt}
        \multirow{2}{*}{ \makecell{SanWen }}   
        &\multirow{2}{*}{ \makecell{9}} &\multirow{2}{*}{ \makecell{Literature}} &Sentences   &10754   &1108    &1376\\
        &                                &                                        &Triples   &12608   &1283    &1560\\
        
    \hline
    \specialrule{0em}{1pt}{1pt}
        \multirow{2}{*}{ \makecell{SciRE }}   
        &\multirow{2}{*}{ \makecell{4}} &\multirow{2}{*}{ \makecell{Scientific}}  &Sentences  &7251    &1067    &1990\\
        &                                &                                        &Triples   &18548   &2778    &5148\\
 
    % \hline
    \bottomrule
\end{tabular}
\vspace{-0.8cm}
\end{table}



\subsection{Baselines}
To investigate the effectiveness of our model, we compare our model with the both character-based and lattice-based variations of the five following models.
%
% \begin{itemize}
%     \item CNN (Zeng et al., 2014) proposes a CNN model for relation extraction.
%     \item PCNN (Zeng et al., 2015) puts forward a piecewise CNN model with multi-instance learning.
%     \item BLSTM (Zhang and Wang, 2015) proposes a bidrectional LSTM model for relation extraction.
%     \item Att-BLSTM (Zhou et al., 2016) is a bidrectional LSTM model with word-level attention mechanism. 
%     \item PCNN+ATT (Lin et al., 2016) improves PCNN model with selective attention mechanism.
%     \item Lattice xxx
%     \item MG-Lattice xx
% \end{itemize}
%
% BLSTM \cite{DongxuZhang2015RelationCV}: A BLSTM model for relation extraction is proposed.
% %
% Att-BLSTM \cite{PengZhou2016AttentionBasedBL}: A BLSTM model with a word-level attention mechanism.
% %
% PCNN \cite{YankaiLin2016NeuralRE}: A segmented CNN model with multi-instance learning was proposed.
% %
% Att-PCNN \cite{JoohongLee2019SemanticRC}: An improved the PCNN model with a selective attention mechanism.
% %
% Basic Lattice \cite{YueZhang2018ChineseNU}: The NER model proposed in 2018 was modified to become a Chinese RE model.
% %
% MG-Lattice \cite{ZiranLi2019ChineseRE}: A model of Chinese RE using multigranular language information and external language knowledge.
% %
% %
% BERT+LSTM \cite{JacobDevlin2022BERTPO}: The encoder is BERT, the LSTM model for the decoder.
% \begin{compactitem}
%     \item BLSTM \cite{DongxuZhang2015RelationCV}: A BLSTM model for relation extraction is proposed.
%     %
%     \item Att-BLSTM \cite{PengZhou2016AttentionBasedBL}: A BLSTM model with a word-level attention mechanism.
%     %
%     \item PCNN \cite{YankaiLin2016NeuralRE}: A segmented CNN model with multi-instance learning was proposed.
%     %
%     \item Att-PCNN \cite{JoohongLee2019SemanticRC}: An improved the PCNN model with a selective attention mechanism.
%     %
%     \item Basic Lattice \cite{YueZhang2018ChineseNU}: The NER model  was modified to become a Chinese RE model.
%     %
%     \item MG-Lattice \cite{ZiranLi2019ChineseRE}: A model of Chinese RE using multigranular language information and external language knowledge.
%     %
%     \item BERT+LSTM \cite{JacobDevlin2022BERTPO}: The encoder is BERT, the LSTM model for the decoder.
% \end{compactitem}
%
For the character-based models, we conduct  experiments with BLSTM \cite{DongxuZhang2015RelationCV}, Att-BLSTM \cite{PengZhou2016AttentionBasedBL}, PCNN \cite{YankaiLin2016NeuralRE} and Att-PCNN \cite{JoohongLee2019SemanticRC},  which utilize traditional neural network  RNN, CNN or Attention mechanism for Chinese relation extraction.
%
% The first four models are commonly used  models.
%
We use DeepKE \cite{NingyuZhang2022DeepKEAD}, an open-source neural network relation extraction toolkit  to conduct the experiments.
%
For the lattice-based models, we compare with Basic-Lattice and MG-Lattice. 
%
In Basic-Lattice \cite{YueZhang2018ChineseNU}, an extra word cell is employed to encode the potential words, and attention mechanism is used to fuse feature,  which can explicitly leverages character and word information. 
%
Moreover, MG-Lattice \cite{ZiranLi2019ChineseRE} models multiple senses of polysemous words with the help of external linguistic knowledge 
%
to alleviate polysemy ambiguity .
%

% \subsection{Evaluation and Implementation details}
%== adamw & setting
%
%
We use Chines BERT-wwm \cite{YimingCui2021PreTrainingWW} as the base semantic encoder for all datasets.
%
We follow the standard evaluation metric and report Precision, Recall, and F1 scores to compare the performance of different models.
%
For each view feature, we implement a linear projection layer with  hidden dim 100.
%
We train our model with the AdamW \cite{IlyaLoshchilov2018FixingWD} optimizer for 50 epochs. 
%
The learning rate is set to 1e-3/5e-5, the batch size is set to 32, 
%
and the model is trained with learning rate warmup ratio 10\% and linear decay.
%
% For all the experiments, we report the averaged metric of 3 runs.
%
\subsection{Experimental Results}
%
To conduct a comprehensive comparison and analysis, we conduct experiments on character-based, lattice-based, multiview-based models on three datasets.
%
% and compare our model with several prior competitive baselines.
%
For a fair comparison,  we implement Basic-MultiView semantic encoder  by replacing the BERT with a bidirectional LSTM and improving the representation of characters using additional bi-word features.
%
In addition, to verify the capability of our method combined with the pretrained model, we choose our method  with the BERT+BLSTM model.

% ============
\begin{table}
\centering
\vspace{-0.8cm}
\caption{F1-scores of Character, Lattice and Multi-View models on all datasets.}
\vspace{0.1cm}
\label{tab: tab2}
\begin{tabular}{p{4cm}|p{3cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}}
% \begin{tabular}{p{3cm}p{3cm}p{1.5cm}p{1.5cm}p{1.5cm}}
% \hline
\toprule
    \multicolumn{2}{c|}{Baseline} &  FinRE & SanWen & SciRE \\
    
    % \hline
    % \multirow{3}{*}{ \makecell{Word-based }}   
    %     &Word-baseline  & 41.23  & 54.26 & xx\\
    %     &+char CNN   &41.60   &56.62  &xx \\
    %     &+char LSTM  &42.20   &56.92  &xx\\
        
 
    % \hline 
    % \multirow{3}{*}{ \makecell{Char-based }}   
    %     &Character-baseline  &40.50   &60.34  & xx\\
    %     &+softword  &41.42   &60.69 & xx\\
    %     &+biword    &40.52   &61.34 & xx\\
    %     % &+softword + biwod &42.03  &61.75  & xx \\
    
    
    \midrule    
        
    % \hline
    \multirow{4}{*}{ \makecell{Character-based }}   
        &BLSTM       &42.87   &61.04   &87.35\\
        &Att-BLSTM  &41.48   &59.48   &88.47\\
        % &CNN         &41.47   &59.42  &xx\\
        &PCNN        &45.51   &81.00  &87.86\\
        &Att-PCNN    &46.13   &60.55  &88.78\\
        
    
    % \hline 
    % \multirow{3}{*}{ \makecell{Multiview-based }}  
    %     &Multiview-based       &xx   &xx & xx\\
    %     &+char                 &xx   &xx & xx\\
    %     &+biword               &xx   &xx & xx\\
    
    \hline
    \specialrule{0em}{1pt}{1pt}
    \multirow{2}{*}{ \makecell{Lattice-based }}   
        &Basic-Lattice  &47.41   &63.88  &89.25\\
        &MG-Lattice     &49.26   &65.61  &89.82\\
    
    
    \hline 
    \specialrule{0em}{1pt}{1pt}
    \multirow{2}{*}{ \makecell{MultiView-based }}  
        &Basic-MultiView     &51.01   &\textbf{68.96}     &90.32  \\
        % &MultiView+char      &xx    &xx  &xx\\
        &MultiView+biword    &\textbf{51.56}    &68.45     &\textbf{91.32}\\
    
    \hline 
    \specialrule{0em}{1pt}{1pt}
    \multirow{2}{*}{ \makecell{MultiView-(BERT)}}  
        &BERT+BLSTM        &51.43    &70.12  &91.25\\
        &BERT+MultiView    &\textbf{53.89}    &\textbf{72.98}  &\textbf{92.18}\\

    % \hline
    \bottomrule
\end{tabular}
\vspace{-0.5cm}
\end{table}

% ===


% =====


% 对于第一列的评价
%
% From the Table \ref{tab: tab2}, we find the following observations. 
% The following observations can be derived from the results shown in the Table \ref{tab: tab2}.
%
We report the main results in Table \ref{tab: tab2}, from which we can observe that:
%
% First, 
% %
% We find that the performance of the lattice-based RE models is better than the performance of the character-based RE models.
% %
% The experimental results show that word-level information enhances the  performance of a character-based model.
%
% First,
(1)
%
The performance of the MultiView-based  model that integrates radical feature and lexicon feature into character-based RE models is notably better than the previous RE baseline models. 
%
This shows our model can leverage the  knowledge from character, radical, and lexicon effectively.
%
% Second,
(2)
%
We observe that our model consistently outperforms the  character-based and lattice-based model on three datasets.
%
% Third,
(3)
%
We can see that the BERT-MultiView outperforms the BERT-BLSTM, which show that the our method can be effectively combined with pre-trained model. 
%
Moreover, the results also verify the effectiveness of our method in utilizing multi-view features  information, which means it can complement the information obtained from the pre-trained model.
%
Based on the experimental results above,
%
it makes sense that integrating different granularity and view information and pre-trained model is beneficial for Chinese RE. 
%

% 


%

%


\subsection{Ablation Studies}
%
We conduct ablation studies to further investigate the effectiveness of the main components in our model on SanWen from two perspectives:  Multi-View Features Encoder Layer and Mixture-of-View-Experts (MoVE) fusion mechanism.

%
\textbf{Effect against  Multi-View Features Encoder Layer}.
%
In this part, we mainly focus on the effect of the different view encoder layer and we conduct following experiment with Basic-MultiView. 
%
We consider three model variants setting:  w/o semantic layer, w/o lexicon layer, w/o radical layer.
%

%================== 进行特征的消融实验

\begin{table}
\centering
\vspace{-0.8cm}
\caption{Precision, Recall, and F1 score on SanWen.}
\vspace{0.1cm}
\label{tab: tab3}
\begin{tabular}{p{5cm}|p{2cm}|p{2cm}|p{2cm}}
% \resizebox{10cm}{15mm}{
    % \begin{tabular}{l|c|c|c}
    % \begin{tabular}{lccc}
    % \hline
    \toprule
         Model  Variant &Precision &Recall  &F1  \\
        % \hline
        \midrule
            Basic-MultiView   &68.55  &67.89  &68.96   \\
        \hline
        \specialrule{0em}{1pt}{1pt}
            \quad w/o Semantic View   &49.47   &53.69  &51.50 \\
            \quad w/o Lexicon View    &64.29    &67.88  &66.04 \\
            \quad w/o Radical View    &66.78    &66.58  &66.68 \\
        % \hline
        \bottomrule
    \end{tabular}
% }
\vspace{-0.5cm}
\end{table}
% ======================== TODO! 分析的时候在文中掺杂数据进行体现
%

As shown in Table \ref{tab: tab3},
%
the performance of our model degrades regardless of which view encoder  removed.
%
The model without semantic layer has the most significant performance drops,  which means that contextual information  between entities is the most important feature in our multi-view encoder.
%
The lexicon features are complementary to  character-based semantic information in different granularity,
%
which also is consistent with previous studies \cite{RuotianMa2020SimplifyTU,CanwenXu2019ExploitingME}.
%
Finally, we are surprised  to find that the less-mentioned radical features, compared to the lexicon feature, appear to bring more benefits.
%
We conclude  that radical information that will give more concrete evidence and show more logic patterns to  the model.
% ====
% Based on the experiment results above,
% 
% It makes sense that multi-view encoder is suitable to alleviate Chinese word segmentation problem and  Chinese character substitution problem because we introduce lexicon and radical features.

%
\textbf{Effect against MoVE Fusion Layer.} 
In this part, we compare three different multi-view fusion strategies: concat (Concat), attention (Attention) and our mixture-of-view-experts (MoVE).
%==================
% \begin{table}
% \centering
% \caption{Effect different feature fusing layer on SciRE.}
% \label{tab: tab1}
% \begin{tabular}{|p{3cm}|p{2cm}|p{2cm}|p{2cm}|}
% \hline
%   Fusion Module     &Precision &Recall  &F1  \\
%     \hline
%         Concat       &x    &xx  &xx\\
%         Attention    &xx   &xx  &xx \\
%         MoVE         &xx   &xx  &xx\\
%     \hline
% \end{tabular}
% \end{table}
% ================ 简单点评一下两个方法
%
The most intuitive way is Concat method, which just put the different view feature together and feed to classifier layer.
%
In order to interact with the information of different views, the existing work  design a fusion layer based on the Attention mechanism \cite{AshishVaswani2017AttentionIA}.
%
As shown in Figure \ref{fig:fig3}(a), we find that the performance of our designed fusion module exceeds Concat 1.2\% and Attention 0.5\% on SanWen, respectively.
%
% This is because the proposed MoVE can adaptively adjust the fusion weight of relevant views according to the characteristics of datasets, which makes the model obtain accurate composite features.
%
This is due to the fact that the proposed MoVE can adapt the fusion weight of relevant views based on the properties of datasets, allowing the model to get appropriate composite features.
%


% ============ vs 融合方式的性能 vs  收敛速度 % % 推理速度 
% \begin{figure}[htbp]
% \vspace{-0.8cm}
% \centering  %居中
%     \subfigure[F1 score.]{   %第一张子图
%     \begin{minipage}{3.5cm}
%     \centering    %子图居中
%     \includegraphics[scale=0.5]{Figures/Figure3/fig3a.pdf}  %以pic.jpg的0.5倍大小输出
%     \label{fig:fig3a}
%     \vspace{-0.5cm}
%     \end{minipage}
%     }
%     % ==============
%     \subfigure[Convergence speed.]{ %第二张子图
%     \begin{minipage}{3.5cm}
%     \centering    %子图居中
%     \includegraphics[scale=0.3]{Figures/todo1.jpeg} 
%     \label{fig:fig3b}
%     \vspace{-0.5cm}
%     \end{minipage}
%     }
%     % ===============
%     \subfigure[Inference speed.]{ %s张子图
%     \begin{minipage}{3.5cm}
%     \centering    %子图居中
%     \includegraphics[scale=0.5]{Figures/fig3c.pdf} 
%     \label{fig:fig3c}
%     \vspace{-0.5cm}
%     \end{minipage}
%     }
    
%     \caption{Compared with different view fusion strategies in F1 score, convergence speed and inference-speed.}    %大图名称
%     \label{fig: fig2}    %图片引用标记
%     \vspace{-0.8cm}
% \end{figure}

% ======================= Latex Figure ====
\begin{figure}
    \begin{tikzpicture}  
            % \tikzstyle{every node}=[font=\small] %<<--- line added
            \hspace*{-1cm} %<<--- line modified for centering
            \begin{tabular}{c@{\hspace{4cm}}c@{\hspace{5cm}}c@{\hspace{cm}}c}
                \begin{axis}  
                    [  
                    width=4.5cm,
                    height=5cm,
                    ybar,
                    bar width=18pt,
                    enlarge y limits=0.15, 
                    enlarge x limits=0.3,
                    legend style={
                        at={(0.5,1.28)}, 
                        anchor=north,
                        legend columns=2,
                        font=\tiny},
                    ylabel= F1 Score.,   
                    ylabel near ticks,
                    ylabel style={
                            at={(-0.18, 0.5)},
                        },
                    xlabel= (a) Performance,
                    % symbolic x coords={(a) F1 Score},  
                    xticklabels=\empty,
                    xtick=data,  
                    nodes near coords,  
                    nodes near coords align={vertical},  
                    % nodes near coords style={anchor=east,rotate=-90,inner xsep=1pt}
                    ]  
                    \addplot coordinates {(Concat,  66.51)  }; 
                    \addplot coordinates {(Attention, 67.12)};  
                    \addplot coordinates {(MoVE, 68.96) };  
                    \legend{Concat, Attention, MoVE} 
                      
                    
                \end{axis}   & 
                \begin{axis}  
                    [  
                    width=5.5cm,
                    height=5cm,
                    legend style={
                             at={(0.5, 1.28)},
                             anchor=north,
                             legend columns=2,
                             font=\tiny
                         },
                    ylabel=Loss.,  
                    ylabel style={
                            at={(0.12, 0.5)},
                        },
                    % enlarge y limits=0.15, 
                    % enlarge x limits=0.1,
                    % ytick={150, 170, 190, 210},
                    xlabel= (b) Convergence speed (Epochs),
                    xticklabels=\empty,
                    % symbolic x coords={, , ,, , , ,, ,, , ,, , },  
                    % xtick=data,  
                    % nodes near coords,  
                    % nodes near coords align={vertical},
                    % bar width=3pt,
                    ]
                \addplot+[line width=1pt, mark size=1pt] coordinates{
                    (0, 207.228)
                    (1, 181.168)
                    (2, 176.251)
                    (3, 171.970)
                    (4, 168.569)
                    (5, 163.827)
                    (6, 160.329)
                    (7, 157.285)
                    (8, 155.415)
                    (9, 152.961)
                    (10, 150.817)
                    (11, 148.469)
                    (12, 147.132)
                    (13, 145.800)
                    (14, 144.970)
                    (15, 143.538)
                    (16, 143.279)
                    (17, 142.468)
                    (18, 142.117)
                    (19, 142.000)
                };
                \addplot+[line width=1pt, mark size=1pt] coordinates{
                    (0, 232.068)
                    (1, 185.107)
                    (2, 171.992)
                    (3, 165.854)
                    (4, 161.866)
                    (5, 157.826)
                    (6, 155.505)
                    (7, 151.831)
                    (8, 149.706)
                    (9, 148.681)
                    (10, 146.518)
                    (11, 145.037)
                    (12, 143.695)
                    (13, 142.993)
                    (14, 142.428)
                    (15, 141.540)
                    (16, 141.059)
                    (17, 140.405)
                    (18, 139.817)
                    (19, 139.800)
                    
                };
                \addplot+[line width=1pt, mark size=1pt] coordinates{
                    (0, 202.286)
                    (1, 164.840)
                    (2, 159.644)
                    (3, 154.772)
                    (4, 152.970)
                    (5, 148.413)
                    (6, 147.322)
                    (7, 144.950)
                    (8, 143.808)
                    (9, 142.668)
                    (10, 141.183)
                    (11, 139.870)
                    (12, 139.557)
                    (13, 139.360)
                    (14, 138.627)
                    (15, 137.758)
                    (16, 137.034)
                    (17, 136.283)
                    (18, 136.069)
                    (19, 135.705)
                    
                };
                % ====
                \legend{Concat, Attention, MoVE} 
                    
                \end{axis}  &
                \begin{axis}  
                    [  
                    width=4.5cm,
                    height=5cm,
                    ybar, 
                    bar width=18pt,
                    enlarge y limits=0.15, 
                    enlarge x limits=0.3,
                    legend style={
                        at={(0.5, 1.28)}, 
                        anchor=north,
                        legend columns=2,
                        font=\tiny},
                    ylabel= Iter/s.,  
                    ylabel near ticks,
                    ylabel style={
                            at={(-0.15, 0.5)},
                        },
                    xlabel= (c) Inference Speed,
                    symbolic x coords={},  
                    xtick=data,
                    ytick={2.5, 2.6, 2.8, 3.0, 3.2},
                    % axis lines= left,
                    nodes near coords,  
                    nodes near coords align={vertical},  
                    ]  
                    \addplot coordinates {(Concat, 3.10) }; 
                    \addplot coordinates {(Attention, 2.63)};  
                    \addplot coordinates {(MoVE, 3.02) };  
                    \legend{Concat, Attention, MoVE} 
                
                \end{axis}  
            \end{tabular}
        \end{tikzpicture} 
    \caption{Compared with different view fusion strategies in Performance, Convergence Speed, Inference Speed.}
    \label{fig:fig3} # 
    \vspace{-0.6cm}
\end{figure}
% ========

A potential concern of our model is that the implementation of MoVE brings additional parameters and increases the complexity of the model.
%
To verify the impact of the MoVE module on the efficiency of our model, 
%
we use the same  hyper-parameters  setting to observe the convergence speed of the model during training and the inference speed during prediction under three different view fusion strategies.
%
As show in Figure \ref{fig:fig3}(b), 
%
with the same training settings, the MoVE helps the model to converge faster and be more stable than Concat and Attention strategies.
%
We attribute this to the ability of MoVE to fuse different view information and filter noise information more effectively, which helps the model to learn more efficiently.
%
Figure \ref{fig:fig3}(c) shows the inference speed.
%
Our MoVE does not reduce the inference speed, because in inference stage the gating structure of MoVE only sparsely activated,
%
and will only leverage information from views that have made significant contributions in the training phase.
%

% ============= 为了验证
%

% \subsection{Case Studies}
% %
% To make it easier to understand how our model works, we visualize two examples on xx(Dataset) in Figure xxx. 
% %
% We find that our xxxs

==> Section/5-Conclusion.tex <==
\section{Conclusion}
% ============= 总结模型
In this paper, we propose a novel multi-view features model for Chinese relation extraction.
%
The proposed model integrates different view representations that fuses semantic,  lexicon  and radical features through a mixture-of-view-expert mechanism.
%
% ============== 总结实验
%
We conduct extensive experiments on three distinct domain datasets and compare our model with several strong baselines. 
%
Experimental results demonstrate that the multi-view Chinese characters can effectively improve the performance for Chinese RE.
%
Furthermore, the ablation studies show  mixture-of-view-expert mechanism  effectively  filters noisy information while improving the efficiency of model training and inference.
%
% ============== 总结未来
% In further work,
In further, 
%
we will consider how to integrate  more knowledge such as part-of-speech, dependency and syntax information and extend it to other language and NLP tasks.
%
\newpage

==> Section/6-acknowledge.tex <==
\section*{Acknowledgments.}
This research was supported partly by the science and technology innovation program of Hunan province under grant No. 2021GK2001.
